Visual-Assisted Sound Source Depth Estimation in the Wild

Depth estimation enables a wide variety of 3D applications, such as robotics, autonomous driving, and virtual reality. Despite significant work in this area, it remains open how to enable accurate, low-cost, high-resolution, and large-range depth estimation. Inspired by the flash-to-bang phenomenon (i.e. hearing the thunder after seeing the lightning), this paper develops FBDepth, the first audio-visual depth estimation framework. It takes the difference between the time-of-flight (ToF) of the light and the sound to infer the sound source depth. FBDepth is the first to incorporate video and audio with both semantic features and spatial hints for range estimation. It first aligns correspondence between the video track and audio track to locate the target object and target sound in a coarse granularity. Based on the observation of moving objects' trajectories, FBDepth proposes to estimate the intersection of optical flow before and after the sound production to locate video events in time. FBDepth feeds the estimated timestamp of the video event and the audio clip for the final depth estimation. We use a mobile phone to collect 3000+ video clips with 20 different objects at up to $50m$. FBDepth decreases the Absolute Relative error (AbsRel) by 55\% compared to RGB-based methods.

==> approach.tex <==
\section{Framework Overview}
Our system contains three key components to realize accurate depth estimation in the wild. The audio visual correspondence module associates visual appearance and sound features of the target object to generate more attention to region of interest (ROI) in frames and audio samples. The visual temporal localization module estimate the moment of collision 

\section{Audio Visual Learning}

\subsection{Audio Visual Correspondence}

\subsection{Video Event localization}

Recent work has focused on localizing the video event at a coarse granularity. The time domain resolution is commonly more than $100$ ms. We further manage to localize the video event at a super resolution of $1$ ms. We explore three different frame consistency from video frames to estimate the potential frame at each millisecond and predict the frame that produces the sound. We first use motion consistency to enable low frame rate video (30 fps) to interpolate and predict high frame rate video (240 fps). The time domain resolution is still more than 4 ms. To further improve the resolution, we take advantage of cycle consistency to enable arbitrary frame prediction. Finally, we forward predict the future frames from low frame rate frames before video event and backward predict frames from frames after video event. We find the most similar frames from the two frame sets, which indicate that the video event happens at this frame.   

\begin{figure}[t]
\centering
\includegraphics[width=0.98\columnwidth]{fig/overall_model.png}
\caption{predict the frame at forward step $t$ based on the frame sequence}
\label{fig:video_model}
\end{figure}

\subsubsection{Supervised learning from motion consistency}

The position of object can keep temporal consistency when the force keeps a temporal consistency. For example, it keeps uniform motion in a straight line when the force is zero. It has the uniform acceleration when the force is constant. The motion consistency breaks down only when there is the impulse force. Thus, we first build the motion model for the temporal consistent motion to predict the collision frame.

The model has a temporal feature extractor to learn the hidden motion embeddings and a frame predictor to map current frame to a new frame with the motion embedding and forward temporal step. The temporal module has a visual extractor to learn the visual features from frames and then feeds into two Bi-GRU layers with 128 hidden neurons. It outputs the motion vector with 32 dimensions encoding current motion features. The frame predictor is a U-Net to perform pixel to pixel mapping. We concatenate the motion embedding and the positional encoding of forward step to the feature vector of unet downsampler and then upsample the features to generate the frame at the given forward step.  The forward step represents the quantity of the frame to predict. It can be set as

\begin{itemize}
    \item integer, for instance, it intends to predict the next frame when forward step is 1.
    \item negative number. it tries to predict previous frame when forward step is -1.
    \item fraction number which is the integral multiples of the ratio of low frame rate to high frame rate. For example, when LFR is 30 and HFR is 240, the forward step can be set as $\frac{1}{8}$ to predict next frame in the HFR video. 
\end{itemize}
Thus, the frame predictor can be noted as 
$$ F_{T + t} = \mathcal{F}(F_{T}, V_{motion}, t) $$ where $F_{T}, V_{motion}, t, \mathcal{F}$ represent the frame at timestamp T, motion embedding, forwarding step and  the trainable U-Net. 
In all, the model can assist the low frame rate video to capture the inherent motion dynamics and predict the frames at the resolutions of high frame rate. We compare the predicted frame with ground truth frame to compute the MSE loss as well as perceptual loss, which is defined as $Loss formulation $. 
    
\subsubsection{self-supervised learning by cycle consistency }
Due to the limited resolution of accessible HFR video, we apply the cycle consistency to learn the arbitrary forward step. After performing the frame prediction with arbitrary forward step $\delta t$, we apply the frame prediction on the predicted frames with forward step $t - \delta t$, where $t$ can still satisfy the constraint of minimal resolution of HFR.  It can be denoted as 
$$ F_{T + t} = \mathcal{F}( \mathcal{F}(F_{T}, \delta t), t - \delta t) $$ 
with this formulation, we enable to predict the frame at any timestamp without the ground truth frame at that frame. The frame sequence can supervise itself to generate the plausible frames. 

\subsubsection{Forward-backward Consistency}

\begin{figure}[t]
\centering
\includegraphics[width=0.98\columnwidth]{fig/forward_backward.png}
\caption{Forward backward estimation and matching to find the most similar frame pair}
\label{fig:forward_backward}
\end{figure}

The collision not only produces the sound but also breaks the motion consistency. The impulse force can change the direction, speed and self rotation of the moving objects. We pick up the frame $F_{before}$ and frame $F_{after}$ as the two nearest frames before and after the collision moment that happens at timestamp $T_col$. We use the frame sequence prior to $F_{before}$ to infer the frames between $F_{before}$ and $F_{after}$ at a high resolution. Meanwhile, we use the frame sequence after $F_{after}$ to infer the frames between $F_{before}$ and $F_{after}$. we compare the two predicted frame to find a pair of most similar frame. The moment of collision is the end of early motion sequence as well as the start of following motion sequence. It is the cross point of two non-overlap trace as the figure~\ref{fig:forward_backward} shows.

\subsubsection{Optical flow matching}

\subsection{Depth Regression in Audio Track}

==> overview.tex <==
\section{System Architecture}
% add the system pipeline figure here
% describe the sketch of each stages;
% flash-to-bang in detail, temporal resolution to depth resolution
\subsection{Optical Flow}
